Decidable Verification of Uninterpreted Programs

We study the problem of completely automatically verifying uninterpreted programs---programs that work over arbitrary data models that provide an interpretation for the constants, functions and relations the program uses. The verification problem asks whether a given program satisfies a postcondition written using quantifier-free formulas with equality on the final state, with no loop invariants, contracts, etc. being provided. We show that this problem is undecidable in general. The main contribution of this paper is a subclass of programs, called coherent programs that admits decidable verification, and can be decided in PSPACE. We then extend this class of programs to classes of programs that are $k$-coherent, where $k \in \mathbb{N}$, obtained by (automatically) adding $k$ ghost variables and assignments that make them coherent. We also extend the decidability result to programs with recursive function calls and prove several undecidability results that show why our restrictions to obtain decidability seem necessary.

==> prelim.tex <==
%!TEX root = main.tex

\section{Preliminaries}
\seclabel{prelims}

We will consider finite first order \emph{signatures} $\Sigma = (\Cc,
\Ff, \Rr)$, where $\Cc$, $\Ff$, and $\Rr$ are finite sets of
constants, function symbols, and relation symbols, respectively. Each
function symbol and relation symbol is implicitly associated with an
arity in $\nats_{>0}$. A first order signature is called
\emph{algebraic} if there are no relation symbols, i.e., $\Rr =
\emptyset$. We will denote an algebraic signature as $\Sigma = (\Cc,
\Ff)$ instead of $\Sigma = (\Cc, \Ff, \emptyset)$. An \emph{algebra}
or \emph{data model} for an algebraic signature $\Sigma = (\Cc, \Ff)$,
is $\Mm = (U, \setpred{\sem{c}}{c \in \Cc}, \setpred{\sem{f}}{f \in
  \Ff})$ which consists of a universe $U$ and an interpretation for
each constant and function symbol in the signature.

Let us fix an algebraic signature $\Sigma = (\Cc, \Ff)$. The set of
(ground) \emph{terms} are those that can be built using the constants
in $\Cc$ and the function symbols in $\Ff$; inductively, it is the set
containing $\Cc$, and if $f$ is an $m$-ary function symbol, and $t_1,
\ldots t_m$ are terms, then $f(t_1,\ldots t_m)$ is a term. We will
denote the set of terms as $\Terms$ (since the signature $\Sigma$ will
be often clear from the context). An equivalence relation $\cong
\subseteq \Terms \times \Terms$ is said to be a \emph{congruence} if
whenever $t_1 \cong t_1'$, $t_2 \cong t_2'$, \ldots $t_m \cong t_m'$
and $f$ is an $m$-ary function then $f(t_1,\ldots t_m) \cong
f(t_1',\ldots t_m')$. Given a binary relation $A \subseteq \Terms
\times \Terms$, the \emph{congruence closure} of $A$, denoted
$\congcl{A}$, is the smallest congruence containing $A$. Inductively,
\begin{itemize}
 \item For every $(t, t') \in A$, $t \congcl{A} t'$
 \item For every function $f$ of arity $m$, and every $2m$ terms $t_1,
   \ldots, t_m, t_1', \ldots t_m'$, if $t_i \congcl{A} t_i'$ for every
   $i \in [1,m]$, then $f(t_1, \ldots, t_m) \congcl{A} f(t_1', \ldots,
   t_m')$.
\end{itemize}
For a congruence $\cong$ on $\Terms$, the equivalence class of a term
$t$ will be denoted by $\eqcl{t}{\cong}$; when $\cong = \congcl{A}$,
we will write this as $\eqcl{t}{A}$ instead of $\eqcl{t}{\congcl{A}}$.

Given a term $t$ and a data model $\Mm$, the \emph{value} that $t$
evaluates to in $\Mm$ will be denoted by $\termsem{t}{\Mm}$. Given a
binary relation $A \subseteq \Terms \times \Terms$, $\Mm$ is said to
\emph{satisfy} $A$ (or $A$ \emph{holds in} $\Mm$) if for every pair
$(t,t') \in A$, $\termsem{t}{\Mm} = \termsem{t'}{\Mm}$.

For a relation $A$, there is a canonical model in which $A$ holds.
%
\begin{definition}
\deflabel{term-model} 
The \emph{initial term model} for $A \subseteq \Terms \times \Terms$
over signature $\Sigma = (\Cc, \Ff)$ is $\termmod{A} = (U,
\setpred{\sem{c}}{c \in \Cc}, \setpred{\sem{f}}{f \in \Ff})$ where
\begin{itemize}
\item $U = \Terms/\congcl{A}$,
\item $\sem{c} = \eqcl{c}{A}$ for any $c \in \Cc$, and
\item $\sem{f}(\eqcl{t_1}{A}, \ldots \eqcl{t_m}{A}) =
  \eqcl{f(t_1,\ldots t_m)}{A}$ for any $m$-ary function symbol $f \in
  \Ff$ and terms $t_1,\ldots t_m \in \Terms$.
\end{itemize}
\end{definition}
%
We conclude this section, by stating an important property of the
initial term model that we will exploit in our results.
%
\begin{proposition}
\proplabel{term-model} 
%
Let $A$ be a binary relation on terms, and $\Mm$ be any model
satisfying $A$. For any pair of terms $t,t'$, if
$\termsem{t}{\termmod{A}} = \termsem{t'}{\termmod{A}}$ then
$\termsem{t}{\Mm} = \termsem{t'}{\Mm}$.
\end{proposition}
%
\begin{proof}
Any model $\Mm$ defines an equivalence on terms $\equiv_{\Mm}$ as
follows: $t \equiv_{\Mm} t'$ iff $\termsem{t}{\Mm} =
\termsem{t'}{\Mm}$. Observe that $\equiv_{\Mm}$ is a congruence, and
if $\Mm$ satisfies $A$, then $A \subseteq \equiv_{\Mm}$. Thus,
$\congcl{A} \subseteq \equiv_{\Mm}$. Next, observe that for the term
model $\termmod{A}$, $\equiv_{\termmod{A}} = \congcl{A}$. The
proposition follows from these observations.
\end{proof}

